Distributionally Adaptive Meta Reinforcement Learning

Meta-reinforcement learning algorithms provide a data-driven way to acquire policies that quickly adapt to many tasks with varying rewards or dynamics functions. However, learned meta-policies are often effective only on the exact task distribution on which they were trained and struggle in the presence of distribution shift of test-time rewards or transition dynamics. In this work, we develop a framework for meta-RL algorithms that are able to behave appropriately under test-time distribution shifts in the space of tasks. Our framework centers on an adaptive approach to distributional robustness that trains a population of meta-policies to be robust to varying levels of distribution shift. When evaluated on a potentially shifted test-time distribution of tasks, this allows us to choose the meta-policy with the most appropriate level of robustness, and use it to perform fast adaptation. We formally show how our framework allows for improved regret under distribution shift, and empirically show its efficacy on simulated robotics problems under a wide range of distribution shifts.

==> texs/algo_pseudocode.tex <==
\section{Algorithmic description of \rml}
\label{sec:algo_code}
    \begin{algorithm}[H]
      	\caption{Meta-training on train and \emph{imagined} test task distribution}
      	\label{alg:train_method}
      	\begin{algorithmic}[1]
      	\STATE Given: $p_{\text{train}}(\gT)$, transition model $\gP$
      	\STATE $\pi_{\theta_1, \epsilon_1}$, Replay Buffer $\gD \leftarrow$ Optimize eq~\ref{eq:meta_train} with $\text{RL}^2$
      	\STATE Optimize eq~\ref{eq:prac_vae} using $\gD$ to obtain task proposer $q_\phi$ and learned reward function $r_\omega$
      	\FOR{$\epsilon$ in $\{\epsilon_2,\ldots,\epsilon_M\}$}
      	    \FOR{iteration $n=1, 2, ...$}
      	        \STATE Optimize meta-RL agent parameter $\theta$ to maximize eq~\ref{eq:gen_robust_meta_train} using $1$ iteration of $\text{RL}^2$.
      	        \STATE Optimize task-distribution proposer's parameter $\phi$ to minimize eq~\ref{eq:gen_robust_meta_train} using $1$ iteration of $1$-step PPO
      	        \STATE Use $1$ step of dual gradient descent to satisfy the constraint $D(q_\phi(\gT) || p(z)) \leq \epsilon$
      	    \ENDFOR
      	\ENDFOR
      	\STATE Returns $\{\pi_{\theta_i, \epsilon_i}\}_{i=1}^M$
      	\end{algorithmic}
    \end{algorithm}

    \begin{algorithm}[H]
    \caption{Meta-agent selection during Meta-test}
      	\label{alg:test_method}
      	\begin{algorithmic}[1]
      	\STATE Given: $p_{\text{test}}(\gT)$, $\{\pi_{\theta_i, \epsilon_i}\}_{i=1}^M$
      	\STATE a = $\mathrm{ones}((M,))$, b = $\mathrm{ones}((M,))$
      	\FOR{iteration $n=1, 2, \ldots, N...$}
      	    \STATE Initialize $\theta = [\beta(a(i), b(i)).\text{sample() } \text{for } i=1:M]$
      	    \STATE Choose $i = \text{argmax}_j \theta_j$
            \STATE Get average success rate $\alpha$ of $\pi_{\theta_i, \epsilon_i}$ on $\{\gT_i\}_{i=1}^T \sim p_{\text{test}}(\gT)$
            \STATE Update $a(i) += \alpha$ and $b(i) += 1 - \alpha$
      	\ENDFOR
      	\end{algorithmic}
    \end{algorithm}
    
    \begin{algorithm}[H]
      	\caption{Meta-training on train and \emph{imagined} test task distribution}
      	\label{alg:train_method}
      	\begin{algorithmic}[1]
      	\STATE Given: $p_{\text{train}}(\gT)$, Return: $\Pi$
      	\STATE $\pi_{\text{meta}, \theta}^{\epsilon_1}$, $\gD_{\text{Replay-Buffer}} \leftarrow$ Solve equation~\ref{eq:meta_train} with off-policy $\text{RL}^2$
      	\STATE Reward distribution $r_\omega$, prior $p(z) \leftarrow$ Solve eq~\ref{eq:prac_vae} using $\gD_{\text{Replay-Buffer}}$
      	\STATE Initialize $\Pi = \{\pi_{\text{meta}, \theta}^{\epsilon_1}\}$
      	\FOR{$\epsilon$ in $\{\epsilon_2,\ldots,\epsilon_M\}$}
      	    \STATE Initialize $q_\phi(z)$, $\pi_{\text{meta}, \theta}^\epsilon$ and $\lambda \geq 0$.
      	    \FOR{iteration $n=1, 2, ...$}
      	        \STATE Update $\theta$ using equation~\ref{eq:theta_grad} with off-policy $\text{RL}^2$
      	        \STATE Update $\phi$ using equation~\ref{eq:phi_grad} with Reinforce
      	        \STATE Update $\lambda$ using equation~\ref{eq:lambda_grad}
      	    \ENDFOR
      	    \STATE Add $\pi_{\text{meta}, \theta}^\epsilon$ to $\Pi$
      	\ENDFOR
      	\end{algorithmic}
    \end{algorithm}

    \begin{algorithm}[H]
    \caption{Meta-policy selection during Meta-test}
      	\label{alg:test_method}
      	\begin{algorithmic}[1]
      	\STATE Given: $p_{\text{test}}(\gT)$, $\Pi = \{\pi_{\text{meta}, \theta}^{\epsilon_i}\}_{i=1}^M$
      	\STATE $\pi_{\text{meta}, \theta}^\epsilon \leftarrow$ $\texttt{Thompson-Sampling}(\Pi, p_{\text{test}}(\gT))$ within $N$ meta episodes.
      	\end{algorithmic}
    \end{algorithm}

==> texs/oos_task_dyn.tex <==
\section{\textcolor{violet}{Evaluations on out-of-support shifted task distributions with varying dynamics}}
\label{sec:oos_task_dyn}
\begin{figure}[H]
    \centering
    \includegraphics[width=0.24\linewidth]{figs/wind.pdf}
    \caption{\textcolor{violet}{\texttt{Wind navigation:} The agent needs to navigate in presence of winds whose velocity $w_\gT$ varies by task}}
    \label{fig:wind_env}
\end{figure}

\textcolor{violet}{
To test \rml~on tasks with varying dynamics, we use the \texttt{wind navigation} environment (controlling a linear system robot in presence of wind, as shown in Figure~\ref{fig:wind_env}) discussed in several prior works on meta-RL~\cite{ni2022recurrent, dorfman2020offline}. In this section, we focus on \textit{out-of-support} shifted test task distributions. To enable \rml~to imagine out-of-distribution dynamics that are out-of-support, we use structured VAE to model dynamics distribution (see Appendix~\ref{subsec:struct_dyn_vae} for more details). Figure~\ref{fig:wind_oos_exps} shows that \rml~matches existing meta RL algorithms ($\text{RL}^2$, VariBAD and HyperX) on training task distribution and outperforms them on shifted test task distributions. Moreover, Figure~\ref{fig:wind_oos_exps} shows that adaptively choosing an uncertainty set during test time allows for better test time distribution adaptation when compared to selecting an uncertainty
set beforehand or selecting a large uncertainty set.}

\begin{figure}[H]
    \centering
    \includesvg[width=0.24\linewidth]{figs/wind_eval_sota.svg}
    \includesvg[width=0.24\linewidth]{figs/wind_eval.svg}
    \caption{\textcolor{violet}{We evaluate \rml~and meta RL algorithms ($\text{RL}^2$, VariBAD and HyperX) on training task distribution and different test task distributions of \texttt{Wind-navigation} environment. \rml~outperforms $\text{RL}^2$, VariBAD and HyperX on train task distribution and different test task distributions. Furthermore, adaptively selecting an uncertainty set for \rml~policy (Adapt) during test time allows it to better adapt to test time distribution shift than choosing an uncertainty set beforehand (Mid). Choosing a large uncertainty set for \rml~policy (Conservative) leads to a conservative behavior and hurts its performance when test time distribution shift is low. The first point $p_1$ on the horizontal axis indicates the training wind speed ($\Delta$) distribution $\mathcal{U}(0, p_1)$ and the subsequent points $p_i$ indicate the shifted wind speed ($\Delta$) distribution $\mathcal{U}(p_{i-1}, p_i)$ (See Table~\ref{tbl:detail_task_dist} for more information on task distributions).}} 
    \label{fig:wind_oos_exps}
\end{figure}

==> texs/visualizing_policies_chosen.tex <==
\section{Visualizing meta-policies chosen by Thompson's sampling}

In this section, we visualize the behavior of different meta-policies (robust to varying levels of distribution shift) towards end of their training. We additionally plot the meta-policies chosen by Thompson's sampling during meta-test phase for different task distribution shifts. We choose \texttt{Ant navigation} task for this evaluation with training task target distance distribution as $\gU(0, 0.5)$ and test task distributions being \textit{out-of-support} of training task distribution (see Table~\ref{tbl:detail_task_dist} for detailed description of these distributions). 

To visualize the behavior of different meta-policies, we extract the $x-y$ position of Ant from the states visited by these meta-policies in their last million environment steps (out of their total $15.2$ million environment steps). We pass these $x-y$ positions through a gaussian kernel and generate visitation heatmaps of the Ant's $x-y$ position, as shown in Figure~\ref{fig:diff_eps_meta_policy}. Figure~\ref{fig:viz_eps} plots the $\epsilon$ values corresponding to meta-policies chosen by Thompson's sampling during meta-test for different test task distributions.

\begin{figure}[H]
    \centering
    \includesvg[width=0.4\linewidth]{figs/gen_ant_goal_eval_epsilon.svg}
    \caption{\textcolor{violet}{$\epsilon$ values corresponding to meta-policies chosen by Thompson's sampling during meta-test for different test task distributions of \texttt{Ant navigation}. The first point $r_{\text{train}}$ on the horizontal axis indicates the training target distance $\Delta$ distribution $\mathcal{U}(0, r_{\text{train}})$ and the subsequent points $r^i_{\text{test}}$ indicate the shifted test target distance $\Delta$ distribution $\mathcal{U}(r^{i-1}_\text{test}, r^i_\text{test})$.}} 
    \label{fig:viz_eps}
\end{figure}

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.2\textwidth}
        \includegraphics[width=\linewidth]{figs/eps/eps_0.0.png}
        \caption{$\epsilon = 0.0$}
    \end{subfigure}
    \begin{subfigure}[b]{0.2\textwidth}
        \includegraphics[width=\linewidth]{figs/eps/eps_0.1.png}
        \caption{$\epsilon = 0.1$}
    \end{subfigure}
    \begin{subfigure}[b]{0.2\textwidth}
        \includegraphics[width=\linewidth]{figs/eps/eps_0.2.png}
        \caption{$\epsilon = 0.2$}
    \end{subfigure}
    \begin{subfigure}[b]{0.2\textwidth}
        \includegraphics[width=\linewidth]{figs/eps/eps_0.3.png}
        \caption{$\epsilon = 0.3$}
    \end{subfigure}
    \begin{subfigure}[b]{0.2\textwidth}
        \includegraphics[width=\linewidth]{figs/eps/eps_0.4.png}
        \caption{$\epsilon = 0.4$}
    \end{subfigure}
    \begin{subfigure}[b]{0.2\textwidth}
        \includegraphics[width=\linewidth]{figs/eps/eps_0.5.png}
        \caption{$\epsilon = 0.5$}
    \end{subfigure}
    \begin{subfigure}[b]{0.2\textwidth}
        \includegraphics[width=\linewidth]{figs/eps/eps_0.6.png}
        \caption{$\epsilon = 0.6$}
    \end{subfigure}
    \begin{subfigure}[b]{0.2\textwidth}
        \includegraphics[width=\linewidth]{figs/eps/eps_0.7.png}
        \caption{$\epsilon = 0.7$}
    \end{subfigure}
    \begin{subfigure}[b]{0.2\textwidth}
        \includegraphics[width=\linewidth]{figs/eps/eps_0.8.png}
        \caption{$\epsilon = 0.8$}
    \end{subfigure}
    \caption{\textcolor{violet}{We visualize the Ant's $x-y$ position visitation heatmaps for different meta-policies towards the end of their training (i.e., in their last $1$ million environment steps, out of $15.2$ million environment steps of training). Here, $\epsilon$ indicates the level of robustness of the meta-policy $\pi_\theta^\epsilon$. The red circle visualizes the training task distribution for \texttt{Ant navigation}.}}
    \label{fig:diff_eps_meta_policy}
\end{figure}
